Validation of Kalman Filter alignment algorithm with cosmic-ray data using a CMS silicon strip tracker endcap

A Kalman Filter alignment algorithm has been applied to cosmic-ray data. We discuss the alignment algorithm and an experiment-independent implementation including outlier rejection and treatment of weakly determined parameters. Using this implementation, the algorithm has been applied to data recorded with one CMS silicon tracker endcap. Results are compared to both photogrammetry measurements and data obtained from a dedicated hardware alignment system, and good agreement is observed.

==> Makefile <==
# Most important - the input file (without .tex extension)
SOURCE     = kalman

# what the Makefile shall produce (choose .ps or .pdf)
TARGET     = $(SOURCE).pdf

######################################################################

#LaTeX, MetaFont, DVIPS and other programs
LATEX      = latex
PDFLATEX   = pdflatex
DVIPS      = dvips
FMFFILE    = f
MF	   = mf
MODE       = \scrollmode

# all TeX sources
TEXSOURCES = $(wildcard *.tex)
TEXSOURCES += $(wildcard tables/*.tex)

# to automatically produce postscript files from feynman graphs
FEYNSOURCE = feynpics
FEYNGRAPHS = $(wildcard fmg/*.fmg)
FEYNEPS    = $(FEYNGRAPHS:.fmg=.eps)

# where to find PostScript (.eps) files to be included
PSPICS     = $(wildcard fig/*.eps)
PSPICS    += $(FEYNEPS)
PDFPICS    = $(PSPICS:.eps=.pdf)


all: $(TARGET)

# main targets

$(SOURCE).dvi: $(TEXSOURCES) $(PSPICS)
	$(LATEX) '$(MODE) \input '"$(SOURCE)" ; while grep -s 'Rerun to get cross-references right' $(SOURCE).log; do $(LATEX) '$(MODE) \input '"$(SOURCE)"; done

$(SOURCE).pdf: $(SOURCE).ps
	pstops "0U(596,29.7cm)" $(SOURCE).ps > $(SOURCE).new.ps 
	ps2pdf -g5960x8430 $(SOURCE).new.ps $(SOURCE).pdf
	rm $(SOURCE).new.ps

$(SOURCE).ps: $(SOURCE).dvi
	$(DVIPS) -o $@ $<

# view

view: $(SOURCE).pdf
	kpdf $< &

# clean

clean:
	rm -rf *.dvi *.lof *.lot *.toc *.bbl *~ *.log *.aux *.blg *.ps *.pdf *.out \
	fig/*~ fig/*.bak fmg/*~ fmg/*.tex fmg/*.log fmg/*.tmp fmg/*.aux

mrproper: clean
	rm -rf $(FEYNEPS) $(PDFPICS)f.*

# rules

fig/%.pdf: fig/%.eps
	epstopdf $< --outfile=$@

fmg/%.pdf: fmg/%.eps
	epstopdf $< --outfile=$@

fmg/%.eps: fmg/%.fmg
	cp $< $<.tex
	echo $< | latex $(FEYNSOURCE) ; rm $(FEYNSOURCE).aux
	$(MF) '\mode:=ljfour; mag:=magstep(4.0); nonstopmode; input $(FMFFILE)'
	mktexpk --mfmode ljfour --bdpi 600 --mag 1+0/600 --dpi 600 f
	echo $< | latex $(FEYNSOURCE)
	dvips -E -o $@ $(FEYNSOURCE).dvi
	rm -rf $(FMFFILE).* $(FEYNSOURCE).{log,aux,dvi} $<.* fmdefault.mf dpi*

